From Library Portability to Para-rehosting: Natively Executing Microcontroller Software on Commodity Hardware

Finding bugs in microcontroller (MCU) firmware is challenging, even for device manufacturers who own the source code. The MCU runs different instruction sets than x86 and exposes a very different development environment. This invalidates many existing sophisticated software testing tools on x86. To maintain a unified developing and testing environment, a straightforward way is to re-compile the source code into the native executable for a commodity machine (called rehosting). However, ad-hoc re-hosting is a daunting and tedious task and subject to many issues (library-dependence, kernel-dependence and hardware-dependence). In this work, we systematically explore the portability problem of MCU software and propose pararehosting to ease the porting process. Specifically, we abstract and implement a portable MCU (PMCU) using the POSIX interface. It models common functions of the MCU cores. For peripheral specific logic, we propose HAL-based peripheral function replacement, in which high-level hardware functions are replaced with an equivalent backend driver on the host. These backend drivers are invoked by well-designed para-APIs and can be reused across many MCU OSs. We categorize common HAL functions into four types and implement templates for quick backend development. Using the proposed approach, we have successfully rehosted nine MCU OSs including the widely deployed Amazon FreeRTOS, ARM Mbed OS, Zephyr and LiteOS. To demonstrate the superiority of our approach in terms of security testing, we used off-the-shelf dynamic analysis tools (AFL and ASAN) against the rehosted programs and discovered 28 previously-unknown bugs, among which 5 were confirmed by CVE and the other 19 were confirmed by vendors at the time of writing.

==> tex/4-case.tex <==
% \begin{table}[t]
%   \centering
%   \caption{Port interface}
%   \begin{adjustbox}{max width=\columnwidth}
%     \begin{tabular}{c|l|l|lr}
%     \toprule
%           & \multicolumn{2}{l|}{\textbf{Module}} & \textbf{UpStream} & \multicolumn{1}{l}{\textbf{DownStream}} \\
%     \midrule
%     \multirow{9}[8]{*}{\textbf{FreeRTOS}} & \multicolumn{2}{l|}{Task Creation} &       & \multicolumn{1}{l}{pxPortInitialiseStack} \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{SysTick} & vTaskSwitchContext &  \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{\multirow{4}[2]{*}{Synchronization}} &       & \multicolumn{1}{l}{portDISABLE\_INTERRUPTS} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{portENABLE\_INTERRUPTS} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{portENTER\_CRITICAL} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{portEXIT\_CRITICAL} \\
% \cmidrule{2-5}          & \multirow{3}[2]{*}{Network (Native)} & Initialization &       & \multicolumn{1}{l}{xNetworkInterfaceInitialise} \\
%           &       & Send  &       & \multicolumn{1}{l}{xNetworkInterfaceOutput} \\
%           &       & Receive & xSendEventStructToIPTask &  \\
%     \midrule
%     \multirow{7}[8]{*}{\textbf{Mbed OS}} & \multicolumn{2}{l|}{Task Creation} &       & \multicolumn{1}{l}{svcRtxThreadNew} \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{SysTick} & osRtxTick\_Handler &  \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{\multirow{2}[2]{*}{Synchronization}} &       & \multicolumn{1}{l}{\_\_disable\_irq} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{\_\_enable\_irq} \\
% \cmidrule{2-5}          & \multirow{3}[2]{*}{Network (LWIP)} & Initialization &       & \multicolumn{1}{l}{low\_level\_init} \\
%           &       & Send  &       & \multicolumn{1}{l}{low\_level\_output} \\
%           &       & Receive & ethernetif\_input &  \\
%     \midrule
%     \multirow{9}[8]{*}{\textbf{Zephyr}} & \multicolumn{2}{l|}{Task Creation} &       & \multicolumn{1}{l}{z\_arch\_new\_thread} \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{SysTick} & z\_reschedule &  \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{\multirow{4}[2]{*}{Synchronization}} &       & \multicolumn{1}{l}{z\_arch\_irq\_lock} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{z\_arch\_irq\_unlock} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{z\_arch\_irq\_disable} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{z\_arch\_irq\_enable} \\
% \cmidrule{2-5}          & \multirow{3}[2]{*}{Network (Native)} & Initialization &       & \multicolumn{1}{l}{ethernet\_api.iface\_api.init} \\
%           &       & Send  &       & \multicolumn{1}{l}{ethernet\_api.send} \\
%           &       & Receive & net\_recv\_data &  \\
%     \bottomrule
%     \end{tabular}%
%     \end{adjustbox}
%     \label{case_study}%
% \end{table}%


% \begin{table}[t]
%   \centering
%   \caption{Port interface}
%   \begin{adjustbox}{max width=\columnwidth}
%     \begin{tabular}{c|l|l|lr}
%     \toprule
%           & \multicolumn{2}{l|}{\textbf{Module}} & \textbf{UpStream} & \multicolumn{1}{l}{\textbf{DownStream}} \\
%     \midrule
%     \multirow{9}[8]{*}{\textbf{FreeRTOS}} & \multicolumn{2}{l|}{Task Creation} &       & \multicolumn{1}{l}{pxPortInitialiseStack} \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{SysTick} & vTaskSwitchContext &  \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{\multirow{4}[2]{*}{Synchronization}} &       & \multicolumn{1}{l}{portDISABLE\_INTERRUPTS} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{portENABLE\_INTERRUPTS} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{portENTER\_CRITICAL} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{portEXIT\_CRITICAL} \\
% \cmidrule{2-5}          & \multirow{2}[2]{*}{Network (Native)}       & Send  &       & \multicolumn{1}{l}{xNetworkInterfaceOutput} \\
%           &       & Receive & xSendEventStructToIPTask &  \\
%     \midrule
%     \multirow{7}[8]{*}{\textbf{Mbed OS}} & \multicolumn{2}{l|}{Task Creation} &       & \multicolumn{1}{l}{svcRtxThreadNew} \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{SysTick} & osRtxTick\_Handler &  \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{\multirow{2}[2]{*}{Synchronization}} &       & \multicolumn{1}{l}{\_\_disable\_irq} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{\_\_enable\_irq} \\
% \cmidrule{2-5}          & \multirow{2}[2]{*}{Network (LWIP)}        & Send  &       & \multicolumn{1}{l}{low\_level\_output} \\
%           &       & Receive & ethernetif\_input &  \\
%     \midrule
%     \multirow{9}[8]{*}{\textbf{Zephyr}} & \multicolumn{2}{l|}{Task Creation} &       & \multicolumn{1}{l}{z\_arch\_new\_thread} \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{SysTick} & z\_reschedule &  \\
% \cmidrule{2-5}          & \multicolumn{2}{l|}{\multirow{4}[2]{*}{Synchronization}} &       & \multicolumn{1}{l}{z\_arch\_irq\_lock} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{z\_arch\_irq\_unlock} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{z\_arch\_irq\_disable} \\
%           & \multicolumn{2}{l|}{} &       & \multicolumn{1}{l}{z\_arch\_irq\_enable} \\
% \cmidrule{2-5}          & \multirow{2}[2]{*}{Network (Native)}      & Send  &       & \multicolumn{1}{l}{ethernet\_api.send} \\
%           &       & Receive & net\_recv\_data &  \\
%     \bottomrule
%     \end{tabular}%
%     \end{adjustbox}
%     \label{case_study}%
% \end{table}%


% \section{Porting}
% \label{sec:specific}

% In this section, we describe the glue layers for Amazon FreeRTOS, ARM Mbed OS, and Zephyr.
% As mentioned earlier, the glue layer only concerns about a
% set of  downstream APIs and a set of upstream APIs.
% Downstream APIs are functions that the glue layer must implement because
% the RTOS core needs to invoke them.
% Downstream APIs are functions provided by the RTOS core.
% They are useful when implementing the Downstream APIs.
% We manually read the source code of these three RTOSs and
% mapped the corresponding downstream and upstream APIs to
% the four modules we abstracted in Section~\ref{sec:abstracing}.
% The results are shown in Table~\ref{case_study}.

  
  
 

% To port FreeRTOS, Mbed OS and Zephyr on \sys,
% we find their hardware model
%   port functions, which are shown in Table~\ref{case_study}.
% We will mainly describe the implementation of Mbed OS port on \sys as an example
% due to most port functions listed in the Table~\ref{case_study}
% designed with similar principles.
% Simultaneously, we will also describe the
% additional or different
% jobs needed to port FreeRTOS and Zephyr.

% \subsection{Mbed OS Task}
% Mbed OS defines the task creation 
% function \texttt{svcRtxThreadNew()}
% to initialise the task control block,
% briefly TCB.
% % \texttt{os\_thread\_t}
% Inside this function,
% Mbed OS initialise the registers' value 
% and store them to stack memory directly,
% instead of implementing them as a port function.
% So we have to replace nineteen lines of code
% with calling \sys thread initialization port function.
% % \texttt{\prefix CreateInstance()}
% Fortunately,
% FreeRTOS and Zephyr have provided 
% the task initialization port functions, as
% shown in Table~\ref{case_study},
% which we just implement them by calling 
% \sys thread initialization port function directly and easily.
% % \texttt{\prefix CreateInstance()}
% \subsection{Mbed OS System Tick}
% All of the RTOSs, including Mbed OS, 
% make use of the \sys system tick
% described in section~\ref{implementation} directly.
% We only need to implement the scheduler glue function
% % \texttt{\prefix SCHEDULER()}
% called by the \sys system tick signal handler.
% % \texttt{\prefix TickSignalHandler()}
% The \sys scheduler glue function
% % \texttt{\prefix SCHEDULER()}
% need to call the Mbed OS scheduler API \texttt{osRtxTick\_Handler()}
% shown in Table~\ref{case_study}
% to store the current task's TCB and reload the next task's TCB,
% both of which will be used
% as identifiers to pair the corresponding thread
% which will be suspended and resumed by the \sys system tick signal handler.
% % \texttt{\prefix SuspendInstance()}
% % and
% % \texttt{\prefix ResumeInstance()}

% \subsection{Mbed OS Synchronization}
% As described in the section~\ref{implementation},
% we need to manage the variable \texttt{\prefix INT\_ENABLED}
% in the glue layer functions.
% Mbed OS defines two functions \texttt{\_\_disable\_irq()} and \texttt{\_\_enable\_irq()},
% as shown in Table~\ref{case_study}, 
% to do this job.
% For FreeRTOS, the critical section port functions 
% \texttt{portENTER\_CRITICAL} and \texttt{portEXIT\_CRITICAL}
% listed in Table~\ref{case_study}
% need to define a variable to count the current task critical section nesting in the glue layer.
% % \texttt{\prefix enter_critical()} and \texttt{prefix exit_critical()}

% \subsection{Mbed OS Network}
% Mbed OS adopts the most popular L3 layer library,
% LWIP~\cite{lwip}, as IP stack implementation, whereas FreeRTOS and Zephyr
% have their own L3 layer implementation.
% But their implementation adopts the same philosophy,
% which is the cornerstone 
% of \sys network port design.

% LWIP declares a network initialization
% port function \texttt{low\_level\_init()}
% as shown in Table~\ref{case_study},
% to initialise the network driver
% and the network interface structure \texttt{netif}.
% We implement this function in the glue layer
% for initialising \texttt{netif} structure
% and calling \sys libpcap initialization port function.
% % \texttt{\prefix LibPcapInitialise()}

% LWIP also declares a packet sending port function \texttt{low\_level\_output()}
% as shown in Table~\ref{case_study}.
% % \texttt{\prefix net_output}
% Inside this glue function,
% we extract the packet buffer pointer and length
% from the structure \texttt{pbuf} and pass them
% to \sys sending packets port function.

% The \sys network initialization port function
% % \texttt{\prefix LibPcapInitialise()}
% creates an anonymous network receiver thread,
% which is not managed as task-thread,
% running a infinite loop 
% to receive packet contiguously.
% In each iteration, 
% the \sys receiving glue function
% is called to receive packets from Ethernet,
% shape them to a specific data structure
% and then deliver them to L3 layer.
% In the \sys receiving glue function,
% we just call the LWIP API \texttt{ethernetif\_input()} directly,
% and \texttt{ethernetif\_input()} will call the LWIP receiving port function \texttt{low\_level\_input()},
% as showed in Table~\ref{case_study}.
% We define the function \texttt{low\_level\_input()} as a macro, whose content is \sys receiving port function.
% Differently, native L3 layer implementation of FreeRTOS and Zephyr
% do not provide the receiving port functions such as \texttt{low\_level\_input()},
% so we must call \sys receiving port function firstly
% in the \sys receiving glue function.

==> tex/9-ack.tex <==
% \section*{Acknowledgments}
% %-------------------------------------------------------------------------------

% The USENIX latex style is old and very tired, which is why
% there's no \textbackslash{}acks command for you to use when
% acknowledging. Sorry.
